Diversifying Anonymized Data with Diversity Constraints

Recently introduced privacy legislation has aimed to restrict and control the amount of personal data published by companies and shared to third parties. Much of this real data is not only sensitive requiring anonymization, but also contains characteristic details from a variety of individuals. This diversity is desirable in many applications ranging from Web search to drug and product development. Unfortunately, data anonymization techniques have largely ignored diversity in its published result. This inadvertently propagates underlying bias in subsequent data analysis. We study the problem of finding a diverse anonymized data instance where diversity is measured via a set of diversity constraints. We formalize diversity constraints and study their foundations such as implication and satisfiability. We show that determining the existence of a diverse, anonymized instance can be done in PTIME, and we present a clustering-based algorithm. We conduct extensive experiments using real and synthetic data showing the effectiveness of our techniques, and improvement over existing baselines. Our work aligns with recent trends towards responsible data science by coupling diversity with privacy-preserving data publishing.

==> extensions.tex <==
\section{$(k,\Sigma)$-Anonymization with Generalization}
\fei{Shall we remove this section, and maybe mention the idea in Conclusion as future work?}
So far we studied $(k,\Sigma)$-anonymization with suppression as the anonymization process. Now, we extend $(k,\Sigma)$-anonymization with generalization. Generalization is an anonymization process that replaces values in a private table with less specific, but semantically consistent values according to a generalization hierarchy~\cite{IYENGARV.S.2002,SAMARATIP.2001,SWEENEYL.2002a, SWEENEYL.2002b,SWEENEYL.1998}. To generalize attribute $A$, we assume a set of levels $\mc{L}^A=\{l^A_0,...,l^A_h\}$ and a partial order $\le^A$, called a {\em generalization relation} on $\mc{L}^A$. Levels $l^A_i$ are assigned with disjoint domain-sets $\dom(l^A_i)$. In $\le^A$, each level has at most one parent. The domain-set $\dom(l^A_n)$ is the maximal domain set and it is a singleton, and $\dom(l^A_0)$ is the {\em ground domain set}. The definition of $\le^A$ implies the existence of a totally ordered hierarchy, called the {\em domain generalization hierarchy}, $\dgh^A$. The domain set $\dom(l^A_i)$ generalizes $\dom(l^A_j)$ iff $l^A_j \leq l^A_i$. We use $h^A$ to refer to the number of levels in $\dgh^A$\ignore{, i.e. $h^A=|\mc{L}^A|$}. 

\begin{figure}[h]
    \centering
    \vspace{-2mm}
    \includegraphics[width=6cm]{./figs/age}
    \vspace{-3mm}
    \caption{(a) \dgh \ and (b) \vgh \ for \att{AGE}.}
    \label{fig:age}
    \vspace{-3mm}
\end{figure}


\begin{definition} [Diversity Constraints with Generalization] \label{df:div-gen} Given a ground relation $R$ with schema $\mc{R}=\{A_1,...,A_n\}$ and generalization hierarchies $\mc{L}^{A_i}$ for each attribute $A_i$, a diversity constraint is a pair $(\sigma,d)$ in which $\sigma$ is a diversity constraint $\nit{floor}\le A_i(a) \le \nit{ceil}$ as in Definition~\ref{df:div} and $d$ is a distance value for values in $\mc{L}^{A_i}$ attribute. A relation $R'$ that generalizes the ground relation $R$ satisfies $\sigma$, denoted by $R' \models \sigma$, if $\nit{floor}\le |\{t\;|\;t \in R', \delta(t[A_i],a) \le d\}| \le \nit{ceil}$. \end{definition}

This means the number of tuples $t$ in $R'$ with value $t[A_i]$ in the distance $d$ of $a$ is at least \nit{floor} and at most \nit{ceil}. The diversity constraints with value generalization extends the diversity constraints with suppression using the distance value $d$ that is a threshold for closeness to a value $a$ to be preserved. 

\fei{This is interesting, but not clear how to incorporate into the algorithm, and also the foundations.  With the above, this sounds more like a starting discussion for future work, where we can define diversity constraints with generalization, and we list the next steps and challenges.}




==> optimization.tex <==
\section{OptimizationZ} \label{sec:opt}

Our optimization of \alg in Algorithm~\ref{alg:diva} targets \nit{DiverseClustering} and its coloring procedure since \nit{Anonymize} (Line~\ref{ln:opt}) is based on an external $k$-anonymization technique.

We optimize \nit{DiverseClustering} by modifying the \nit{Coloring} procedure to run in parallel. The parallel coloring procedure consists of three phases. In the first phase, the set of vertices of graph $G$ is partitioned into $p$ blocks as ${\Gamma_1, ... ,\Gamma_p}$. The objective in this partitioning is to place vertices (constraints) with overlapping target tuples in the same block and make sure the vertices in different blocks have minimum overlap. The vertices in each block are then colored in parallel using $p$ processors and running Algorithm~\ref{alg:coloring}. The synchronization is done at the end of this step. In doing so, two processors may attempt to color adjacent vertices (find clusterings for their constraints) which results to inconsistent clusterings. In the second phase, each processor $p_i$ checks whether vertices in $\Gamma_i$ are assigned consistent clusterings by comparing their vertices against all its neighbors that are in
the other blocks. This checking is also done in parallel. Finally, in the
third phase, the inconsistent vertices that are discovered in the previous step are colored sequentially.

%\fei{Suppression is not discussed in detail in the previous section, and Optimal clustering sounds as if any $k$-anonymization alg. will do.  Is this correct?}

%\subsection{Distributed Clustering}\label{sec:distributed}

%The runtime of \nit{ExistsClustering} depends \nit{NextConstraint} and the order in which the next constraints are considered in Line~\ref{ln:next} (cf. Algorithm~\ref{alg:coloring}). This is analogous to choosing the next vertex to color in the graph coloring problem where several heuristics are presented, e.g. choosing the vertex with the highest degree or the vertex with the fewest possible colors.  \fei{Sounds like this needs more discussion on selection strategy of next $\sigma$.}

\ignore{We propose two optimizations to improve \alg performance. First, we optimize the computation of consistent sets of clusters. The final consistent sets of clusters in $\mathbb{U}$ is not influenced by the order of evaluation of the diversity constraints.  However, this evaluation order can impact the running time of \alg. The number of clusterings in $\mathbb{U}$ can grow exponentially w.r.t. $|\Sigma|$ even if many of these clusterings are pruned due to inconsistencies (e.g., in Example~\ref{ex:alg}, $|\mathbb{U}|$ increases from 0 to 15, and then decreases to 1). In this optimization, we sort the diversity constraints in $\Sigma$ by $\frac{M}{k} \times \binom{N}{k}$ with $M=(\nit{ceil}-\nit{floor})/2$ and $N=|R[A=a]|$, which is an estimation of the number of clusterings in $\mathbb{U}_\sigma$. In the second optimization, we reduce the number of consistent sets of clusters by removing those sets in $\mathbb{U}$ that are dominated by an existing consistent set of clusters. We say $\mc{S}_1 \in \mathbb{U}$ dominates $\mc{S}_2 \in \mathbb{U}$ if for every cluster $C_2 \in \mc{S}_2$ there is a cluster $C_1 \in \mc{S}_1$ and $C_2 \subseteq C_1$ which indicates $\mc{S}_1$ will satisfy $\Sigma$ with a fewer number of suppressed values compared to $\mc{S}_2$, thereby making $\mc{S}_2$ redundant.

The worst-case running time of Algorithm~\ref{alg:CDPG} depends on (i) the number of iterations in the for loop (line~\ref{l:for}) that is the number of possible pairs of clusters at each step of the algorithm, and (ii) the cost of computing utility in line~\ref{l:cgu}. To scale-up the algorithm, we try to optimize with respect to both (i) and (ii). The optimized algorithm is shown in Algorithm~\ref{alg:opt}.

For (i), we apply an optimization that reduces the number of candidate cluster pairs in line~\ref{l:for} of Algorithm~\ref{alg:CDPG}. The idea is to store and use additional data in a map $\mc{M}$. For each cluster $c \in \mc{C}$, $\mc{M}[c]$ contains $q$ closest clusters to $c$ w.r.t. the according to the following distance function,

\vspace{-5mm}
\begin{align}
\nit{dist}(c,c')=\nit{penalty}(c\cup c').\label{frm:cdist}
\end{align}

\noindent The algorithm computes the clusters in $\mc{M}$ in line~\ref{l:initM} and updates it in line~\ref{l:updateM} after the algorithm changes the current clustering $\mc{C}$. The optimized algorithm uses $\mc{M}$ in line~\ref{l:foro} to iterate over a reduced number of candidate clusters.

\begin{example} (ex.~\ref{ex:alg} cont.) The for loop in Algorithm~\ref{alg:CDPG} runs 28 times for different pairs of clusters from $c_1,...,c_8$. In Algorithm~\ref{alg:opt} and assuming $q=2$, $\mc{M}[c_1]=\{c_2,c_3\}$ with $c_2$ and $c_3$ as the closest clusters to $c_1$. This will reduce the number of pairs to consider from 28 to $|\mc{C}| \times q = 8 \times 2=16$.\end{example}

To decrease the cost of computing the utility measure, we use a map $\mc{U}$ that stores for each pattern $p \in R_g[F]$, the clusters with maximum preserve measure. That means each $c_p \in \mc{U}[p]$ is a cluster with maximum value of $\nit{preserve}(c_p,p)$. We compute the utility of a new clustering $\mc{C}_{i,j}$ using $\mc{U}$. Let $P=\{p_{1},p_{2}, \cdots\}$ represent the patterns in the clusters $c_{i}$ and $c_{j}$.  For each pattern $p\in P$, we consider two cases after merging $c_i$ and $c_j$. 

\begin{itemize}
\item $\nit{preserve}(c_{i,j},p) \ge \nit{preserve}(c_p,p)$: The utility value is computed with new preserve for $p$, i.e. $\nit{preserve}(c_{i,j},p)$.
\item $\nit{preserve}(c_{i,j},p) < \nit{preserve}(c_p,p)$: If $\mc{U}[p] \setminus \{c_i, c_j\} \neq \emptyset$, which means either $c_i,c_j$ are not in $\mc{U}[p]$ or they are not the only ones in $\mc{U}[p]$ and the utility value can be computed with the past preserve value for $p$, i.e. $\nit{preserve}(c_p,p)$, since it is still the maximum preserve. If $\mc{U}[p] \setminus \{c_i, c_j\} = \emptyset$, we need to search between all the clusters to find the one with new maximum preserve.
\end{itemize}

Using $\mc{U}$, computing the utility measure can be done in $O(|P|)$ in best-case when no search is needed to find the best cluster for a pattern, and $O(|P| \times |R|)$ in worst-case when we need to always search as the best cluster is always merged. This reduces the initial running time of $O(|P| \times |R|)$ for both worst-case and best-case. The optimized algorithm computes $\mc{U}$ initially for the singleton cluster $\mc{C}$ (line~\ref{l:initU}) and updates it as $\mc{C}$ gets updated (line~\ref{l:updateU}). The data in $\mc{U}$ is used in line~\ref{l:cguo} to compute the CGP values.


\begin{algorithm}

\KwIn{Private relation $R$, set of FDs $\Pi$, value $k$.
}

\KwOut{A $k$-anonymous generalization of $R$ that preserves dependencies of $\Pi$.}

\vspace{2mm}
$S := \emptyset$; $\;\;\mc{C}=\emptyset$; \label{l:init}

%\tcc*[h]{\small Tuples with sealed clusters}\label{l:init1}

 %\tcc*[h]{\small Current clustering}\label{l:init2}

\vspace{2mm}
%\tcc*[h]{\small Initialize $\mc{C}$ with a cluster for every tuple}

\ForEach {{\bf tuple} $t_{i} \in R$} {
	$\mc{C} \leftarrow \mc{C} \cup \{ \{ t_i \} \}$;
}

$\mc{M} := \nit{findNearestClusters}(\mc{C})$;\label{l:initM}

$\mc{U} := \nit{findBestClusters}(\mc{C})$;\label{l:initU}

\vspace{2mm}
\While{$|R \setminus S| \ge k$ \label{l:whileo}}
{
$\nit{MaxU} := 0$;  $\;\;\mc{C}':=\emptyset$; 

%\tcc*[h]{\small Maximum utility}  \tcc*[h]{\small Next clustering with maximum utility}

\ForEach {$c_{i} \in \mc{C}$ {\bf and} $c_{j} \in \mc{M}[c_i]$  \label{l:foro}}
      {
      	$c_{i,j} := \nit{merge}(c_i,c_j)$; 
        
        $\mc{C}_{i,j} := (\mc{C} \setminus \{c_i, c_j\}) \cup \{c_{i,j}\}$;
        

        \If{$|c_i\cup c_j| > k$} {
        	$c' := (c_i \cup c_j) \setminus c_{i,j}$; $\;\;\mc{C}_{i,j} := \mc{C}_{i,j} \cup \{c'\}$;
        }
		

        $u := \nit{OPCGU}(\mc{C}_{i,j},R,\Pi,\mc{U})$; \label{l:cguo}

        \If{$u > \nit{MaxU}$} {
        	$\nit{MaxU} := u$; $\;\;\mc{C}' := \mc{C}_{i,j}$;
        }
	  } 

      \ForEach { {\bf cluster} $c$ {\bf in}  $\mc{C}' \setminus \mc{C}$ \label{l:iseal}}
      {
      	\lIf{$|c| = k$} {$S := S \cup c$}
      }

      $\mc{C} := \mc{C}'$;           
      
      $\mc{M} := \nit{updateNearestClusters}(\mc{C},\mc{M})$; \label{l:updateM}
      
      $\mc{U} := \nit{updateBestClusters}(\mc{C},\mc{U})$;\label{l:updateU}
}

\KwRet{$R^\mc{C}$};
\caption{OPTCDPG($R$, $\Pi$, $k$)}\label{alg:opt}
\end{algorithm}



\begin{example} (ex.~\ref{ex:alg} cont.) After computing $\nit{utility}(\mc{C})=3$, we initialize $\mc{U}$ for the 6 patterns in $R_g$. For example for $p_1=({\sf V6J}, {\sf BC})$, $\mc{U}[p_1]=\{c_1,c_2\}$ . Merging $c_1,c_2$ decreases the minimum penalty and we can recompute CGP simply by replacing the value of $\nit{penalty}(p_1,c_1)$ with $\nit{penalty}(p_1,c_{1,2})$; \blue{Merging $c_1,c_3$  or $c_2,c_3$ results to the same penalty obtained from $c_2$ since the minimum penalty for $p_1$ does not change} \end{example}

\begin{comment}
\purple{\Harika: clusters $c_1 \cdots c_4$ are not singleton acc. to Example 4.2.}
\purple{Harika: Highlighted sentence is not clear}.
\end{comment}}








==> problem.tex <==
\section{The $(k,\Sigma)$-Anonymization Problem}\label{sec:problem}

To capture diversity, we define a set of declarative \emph{diversity constraints} that specify lower and upper bounds on the number of attribute values in a published relation. 


%\begin{itemize}
 %   \item Fixed bound: \red{$\att{CITY}:3\le \val{Calgary} \le 12$ or $3\le \att{CITY}[\val{Calgary}] \le 12$}
    %\item Variable bound: \red{$\att{CITY}:c(..)\le \val{Calgary} \le f(...)$}
%\end{itemize}




%\vspace{2mm} \noindent \textbf{Diversity Constraints.} Diversity in an anonymised instance requires the anonymized relation to have a minimum or a maximum representation of some specific group of individuals. For example, a data publisher may prefer a $3$-anonymous relation with geographical diversity containing at least $3$ and at most $12$ patients from \val{Calgary}. We represent this with a {\em fixed-bound diversity} constraint where the minimum and maximum number of values are captured by {\em ceiling} and {\em floor} as fixed multiple of $k$, e.g. $3\le \att{CTY}(\val{Calgary})\le 12$.  In different application, the ceiling and lower bounds in a diversity constraint are often not a fixed number and depend on the total number of revealed value (non-$\star$). For example, a diversity constraint requires between $45\%$ and $55\%$ of the revealed gender values to be \val{Female}. Note that the number of revealed genders is not a fixed and known number. We capture this constraint with {\em variable-bound diversity constraints}, e.g. $0.45 \times c \le \att{GEN}(\val{Female})\le 0.55\times c$ in which $c$ is the number of non-$\star$ values in the published relation. 


To express these constraints, we adopt the definition of diversity constraints in~\cite{fairness} for relational data. In~\cite{fairness}, diversity constraints are used for {\em the set selection problem} that require diverse values among a selected set of top-$m$ items. 

%They propose these constraints for selecting items with diverse attribute values in the set selection problem, i.e. the problem of selecting top $m$ items based on some score. We adapt these constraints for attributes in relational data.

\begin{definition} [Diversity Constraints] \label{df:div} Consider a $k$-anonymous relation $R'$ with schema $\mc{R}$. We define two types of diversity constraints (the latter is a more general form of the former):

\begin{itemize}
    \item{\bf Fixed-bound constraint}: a fixed-bound constraint is of the form $\nit{floor} \le \nit{count}(R'[A],a) \le \nit{ceiling}$ in which $A \in \mc{R}$, $a \in \nit{dom}(A)$, $\nit{count}(R'[A],a)$ is the number of times the value ``$a$'' appears in $R'[A]$, and \nit{floor} and \nit{ceiling} are multiples of $k$.
    \fei{Why tie the lower and upper bound to k-anonymity? I'm hesitant to do this as it limits its general applicability.}
    \mostafa{This is not really a limitation and is only for making constraints more clear. For example, if $k=3$ then $2 \le \nit{count}(R'[A],a) \le 7$ and $1 \le \nit{count}(R'[A],a) \le 8$ have the same effect as $3 \le \nit{count}(R'[A],a) \le 6$ because $\nit{count}(R'[A],a)$ is a multiple of $k$ anyways and can not be 2, 7 and 8.}
    \fei{I understand.  However, this is assuming that the revealed values are only in QI attributes (a restriction of k-anonymity), and that each cluster is exactly size $k$.  If I have a minimum cluster size of $k$, can I not get values in $R'$ that are non-multiples of $k$?}
    
    \item{\bf Variable-bound diversity constraint}: a variable-bound diversity constraint is of the form $f(...) \le \nit{count}(R'[A],a) \le c(...)$ in which $c(...)$ and $f(...)$ are functions of $|R'|$ (the number of tuples in $R'$) and $\nit{count}(R'[A],\star)$ (the number of $\star$'s in $R'[A]$), and return multiples of $k$.
\end{itemize} A diversity constraint $\sigma$, fixed- or variable-bound, is satisfied by $R'$ denoted by $R' \models \sigma$ if and only if $\sigma$ holds as a mathematical inequality according to the attribute values in $R'$.\boxtheorem\end{definition}  

The bounds in diversity constraints enables us to specify anonymized relations with diverse values. These constraints impact the anonymization process to generate these diverse values. Clearly, this is only possible if the initial relation contains diverse values which means the diversity constraints are only indirectly affected by the initial relation; they impose restrictions solely on the anonymized relation.  Variable-bound constraints extend fixed-bound constraints by allowing bounds that depend on the total number of anonymized values ($\star$'s) and revealed values (non-$\star$'s). These are not fixed and can change during the anonymization process and therefor can not be expressed with fixed-bound constraints.
%\fei{Let's discuss: a(A), $\phi$ to $\sigma$, extension? similar notation as [5]?}

\begin{example}\em \label{ex:div} In Example~\ref{ex:intro}, $\sigma_1: 3 \le \nit{count}(R_1[\att{ETH}], \val{Asian}) \le 6$ is a fixed-bound diversity constraint over $R_1$ that requires at least 3 and at most 6 tuples with \val{Asian} ethnicity and is falsified by $R_1$ in Table~\ref{tab:r1} because there is no such ethnicity in $R_1$. A similar constraint $3 \le \nit{count}(R_2[\att{ETH}], \val{Asian}) \le 6$ is satisfied by $R_2$ in Table~\ref{tab:r2} that contains exactly $3$ Asians. A diversity constraint might have a missing upper or lower bound. For example, $3 \le \nit{count}(R_1[\att{ETH}], \val{Asian})$ is a valid diversity constraint that requires $R_1$ to have at least 3 Asians and does not impose an upper bound.

The following is a variable-bound diversity constraint that requires at least $30\%$ of the revealed genders in $R_1$ to be females: $\nit{f}(...) \le \nit{count}(R_1[\att{GEN}],$\ $\val{Female})$ with $\nit{f}(...)=\ceil{0.3 \times |R_1|-\nit{count}(R_1[\att{GEN}],\star)}_k$ ($\ceil{x}_k$ rounds $x$ to the first greater multiple of $k$, e.g. $\ceil{0.9}_3=3$ and $\ceil{4.9}_3=6$). $R_1$ falsifies the constraint because $f(...) = \ceil{0.3 \times 9 - 6}_3 = \ceil{0.9}_3 = 3$ and $R_1$ does not contain any female. Note that $|R_1|-\nit{count}(R_1[\att{GEN}],\star)$ is the number of tuples with a revealed gender value. $R_2$ in Table~\ref{tab:r2} satisfies a similar diversity constraint because it contains three females.

Diversity constraints can be extended to multiple attributes, e.g. $3 \le \nit{count}(R_2[\att{GEN},\att{ETH}],(\val{Female},\val{Asian}))$ is a fixed-bound diversity constraint that requires at least $3$ Asian females in $R_2$. Here,  $\nit{count}(R_2[\att{GEN},\att{ETH}],$ \ $(\val{Female},\val{Asian}))$ counts the number of times \val{Female} and \val{Asian} co-occur in the same tuple in $R_2$.\boxtheorem\end{example}
%restrict to least 3 and at most 4 females, and at least 3 and at most 5 African individuals

%\noindent \textbf{Problem Definition.}  We now formally define our problem.
%that finds a $k$-anonymous instance satisfying a set of diversity constraints $\Sigma$.

\vspace{2mm}
%\noindent {\bf Fairness Constraints.} The notion of fairness, as we briefly explained in Example~\ref{ex:intro}, is essentially different from diversity. The diversity constraints in Definition~\ref{df:div} are defined for an anonymized relation and are independent of the initial input relation. However, fairness is about the closeness of the distribution of values in the input relation and the anonymized output relation. For example, a data publisher might want the same ratio of female to male in the anonymized relation and the input relation. To define these fairness semantics in PPDP, we adapt the fairness constraints for set selection~\cite{fairness}.

\begin{definition} [Fairness Constraints] \label{df:div} Consider a relation $R$ with schema $\mc{R}$ and a $k$-anonymous relation $R'$ with the same schema such that $R\sqsubseteq R'$. A {\em fairness constraint} is of the form $\eta: \nit{f}(...) \le \nit{count}(R[A],a) \le \nit{c}(...)$ in which $\nit{f}(...)$ and $\nit{c}(...)$ are functions of $|R'|$, $\nit{count}(R'[A],\star)$ and $\nit{count}(R[A], a)$. $\langle R, R'\rangle\models \eta$ when $\eta$ holds as an inequality considering the values in $R$ and $R'$.\boxtheorem\end{definition}  

Fairness constraints extend variable-bound constraints by allowing bounds that depend not only on anonymized relation $R'$ but also the initial relation $R$ (in particular $\nit{count}(R[A],a)$). This enables the fairness constraints to compare the distribution of values in the two relations. Fairness, as a general requirement, is usually interpreted as having an anonymized relation with similar distribution of values to the distribution of values in the initial relation. This can be expressed by the fairness constraints.

\begin{example} The fairness constraint $f(...) \le \nit{count}(R_2[\att{GEN}],$ \ $\val{Female})$ with $f(...)=\ceil{p \times (|R_2|-\nit{count}(R_2[\att{GEN}],\star)}_3$ requires at least $p\%$ of the revealed genders in $R_2$ to be \val{Female} in which $p$ is the percentage of females in the initial relation $R$ (note that $|R|=|R_2|$):  

\vspace{-3mm}
\begin{align*}p=\frac{\nit{count}(R[\att{GEN}], \val{Female})}{|R|}\end{align*}

\noindent According to the data of $R$ and $R_2$ in Tables~\ref{tab:r} and \ref{tab:r2}, resp., $\langle R,R_2 \rangle$ satisfy this fairness constraint. That is because $f(...)=\ceil{4/9 \times (9 - 6)}_3=\ceil{4/9 \times (9 - 6)}_3=3$ and there are exactly $3$ females in $R_2$.\boxtheorem\end{example}

\noindent \textbf{Problem Statement.} 
\begin{definition}[$(k,\Sigma)$-anonymization] \label{df:pr} Consider a relation $R$ of schema $\mc{R}$, a constant $k$, a set of constraints $\Sigma=\Sigma_1\cup\Sigma_2$ with diversity constraints $\Sigma_1$ and fairness constraints $\Sigma_2$. The {\bf $(k,\Sigma)$-anonymization problem} is to find a relation $R^*$ that has the following properties: (1) $R \sqsubseteq R^*$, (2) $R^*$ is $k$-anonymous, (3) $R^* \models \Sigma_1$, (4) $\langle R, R^*\rangle \models \Sigma_2$, and (5) $R^*$ has minimal information loss, i.e., minimum number of $\star$'s.
\boxtheorem\end{definition}


\noindent \textbf{Complexity Analysis.} 
The $(k,\Sigma)$-anonymization problem is NP-hard because it generalizes the $k$-anonymization problem with diversity and fairness constraints in $\Sigma$. 
%The following theorems prove the complexity of the satisfiability problem for $(k,\Sigma)$-anonymization.  



%\fei{The last part of this sentence sounds as if we are just adopting an existing algorithm [14], with little novelty.  Can we re-phrase this to sound more novel?}

%\begin{proposition} The $(k,\Sigma)$-anonymization problem is NP-hard and the $(k,\Sigma)$-anonymization decision problem is in PTIME.\end{proposition}

 %\fei{sub-optimal, can we be more specific, does not sound appealing}

\ignore{\begin{table}[h]
\begin{center}
\normalsize
\setlength\tabcolsep{2 pt}
\vspace{-3mm}
%\scalebox{0.9}{
\begin{tabular}{ | l | l | l | l || l | l | l |}
\hline
 \textbf{ID}  &  \textbf{PC}    &  \textbf{PRV} &  \textbf{GEN} &  \textbf{DIAG} &  \textbf{MED}  \\
\hline \hline
$t_1$  &   {\bf R7A} &  {\bf AB} & *  &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_2$  &   {\bf R7A} & {\bf AB} & * &  {Osteoarthritis} & {Naproxin}\\
\hline
%$t_5$  &   K2H & ON & Female &  seizure & diazepam\\ \hline
%$t_6$  &    J5B & QC & Female &  seizure & diazepam\\ \hline
$t_3$  &    {\bf R7A}  & {\bf MB} & * &  {Osteoarthritis} & {Naproxin}\\
\hline
$t_4$  &    {\bf R7A}  & {\bf MB} & * &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_6$  &    J5B & QC & {\bf Male} & {\bf Seizure} & {\bf Diazepam}\\
\hline
$t_7$  &    J5B & QC & {\bf Male} & {\bf Seizure} & {\bf Digoxin}\\
\hline
\end{tabular}
\vspace{0mm}
\caption{General and inconsistent relation $R_1$}
\label{tab:r1}
\end{center}
\end{table}}

\ignore{\begin{figure}[h]
\begin{center}
%\vspace*{-4mm}
\includegraphics[width=7cm]{./figs/figs.pdf}
%\vspace*{-4mm}
\caption{\vghs of (a) PRV and (b) MED.}\label{fig:general}
\end{center}
\end{figure}}

\ignore{A private relation in PPDP can be subject to some integrity constraints (ICs) to keep its data consistent. These constrains might be falsified by the private relation for different reasons such as the integration of data from conflicting sources, faulty data entry, or data staleness. In $R$, we assume two simple ICs in form of FDs $\varphi_{1}: \nit{PC} \rightarrow \nit{PRV}$ and $\varphi_{2}: [\nit{GEN},\nit{DIAG}] \rightarrow \nit{MED}$ that are falsified by $t_1$-$t_4$ and $t_7,t_8$, respectively (error values in bold). A public general relation in PPDP might inherit this inconsistency from its private relation as this happened in $R_1$. In this work, we would like to define the data consistency in the public relation as the third objective in PPDP.}

\ignore{\begin{table}[h]
\begin{center}
\normalsize
\setlength\tabcolsep{2 pt}
%\scalebox{0.9}{
\begin{tabular}{ | l | l | l | l || l | l | l |}
\hline
 \textbf{ID}  &  \textbf{PC}    &  \textbf{PRV} &  \textbf{GEN} &  \textbf{DIAG} &  \textbf{MED}  \\
\hline \hline
$t_1$  &   R7A &  Prairies & Female  &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_2$  & R7A & Prairies & Male &  {Osteoarthritis} & {Naproxin}\\
\hline
%$t_5$  &   K2H & ON & Female &  seizure & diazepam\\ \hline
%$t_6$  &    J5B & QC & Female &  seizure & diazepam\\ \hline
$t_3$  & R7A & Prairies & Male &  {Osteoarthritis} & {Naproxin}\\
\hline
$t_4$  & R7A & Prairies & Female &  {Osteoarthritis} & {Ibuprofen}\\
\hline
$t_6$  &    J5B & QC & Male & Seizure & Anesthetics\\
\hline
$t_7$  &    J5B & QC & Male & Seizure & Anesthetics\\
\hline
               \end{tabular}
\caption{\small General and consistent relation $R'$}
\label{tab:r2}
\end{center}
\end{table}}

\ignore{To publish a consistent version of an inconsistent private relation, we can repair the relation before publishing it. However, it might be preferable to integrate data repair with the data generalization process. This is mainly because data repair is usually costly and it can only be applied to a limited number of errors in an error prune and inconsistent private relation while some of the repaired values might be generalized and detracted in the generalization process for data publishing. For example, $R_2$ in Table~\ref{tab:r1} is a public $k$-anonymous version of $R$ that generalizes AB and MB to Prairies. If we decide to publish $R_2$ there is no point in repairing $t_1$-$t_4$ by updating AB to MB which might be expensive to figure out while it will be distorted anyway during the generalization process. This generalization masks the violation of $\sigma_1$ and it can be seen as a form of data repair.  This basically shows by integrating data repair and the generalization process, we have to ways to resolve inconsistency in a private relation, either by repairing them (e.g. AB to MB in case we decide to publish $R_1$) or by masking the errors thought value generalization. Assuming a limited resources for data repair, we can balance between these two to obtain a consistent and general relation. For example, if there is only one value repair can be done in $R$, we can resolve errors in $t_1$-$t_4$ through generalization and save this repair to fix $t_6$, e.g. Diazepam to Diagoxin which will not be detracted and will be published.  }

\ignore{Based on the discussion above, we define the problem of consistent data publishing as follows. Consider a relation $R$ of schema $\mc{S}$ with a set of QIs $A_1,...,A_n$ and sensitives $B_1,...,B_m$ and a set of FDs $\Sigma$. Let $\nit{cost}_\Sigma(.)$ be a function that specifies the cost of repairing a relation of schema $\mc{S}$ w.r.t. $\Sigma$, $\nit{loss}(.)$ be function that measures of information loss in a relation of $\mc{S}$, and let $B$ be a fixed repair budget. The problem is to find a public relation $R'$ of schema $\mc{S}$ that satisfies the followings: 

\begin{enumerate}
    \item $R'$ generalizes $R$,
    \item it is $k$-anonymous,
    \item $\nit{cost}_\Sigma(R') \le B$,
    \item $R'$ has minimum $\nit{loss}( R')$.
\end{enumerate}}

%\mostafa{Here I defined the problem using a single cost function and not a cost model for each repair operation. I did this because I did not want to get involved with how repair is done and what repair operations are.}


%\fei{Or as we discussed, it may just mask an error, which may not be satisfactory either.} \mostafa{We can cite~\cite{solmaz} as a similar repair technique to justify this way of repair.} 

%Third, the usefulness of the repaired values in a private relation depends on the accuracy of the applied repair algorithms. For example, a repair algorithm might update MB in $t_3$ and $t_4$ to AB to resolve the inconsistency while we know R7A is actually a postal code in MB. These are reasons that someone might choose $R_2$ that resolves the FD violation by generalization rather than application of a separate repair algorithm.  \fei{Yes, but this point requires known semantics between PC and PRV, which we are not providing in this proposed work right?  There is a fundamental assumption here that the dirty data values are somewhat close, albeit inconsistent, in order for your Prairies repair to work.  If the dirty data values are ``far apart'' then generalization does not provide added value.}

%\fei{I would add a point that given limited cleaning resources, it is not always possible to clean a large number of cells, we must be selective due to finite resources, which we can model via a budget.} 
%\blue{This might have different reasons. First, the repair algorithms usually have limited cleaning resources and can not repair large number of cells and therefore it might not be possible to repair every cell in a private database.}  Second, repairing some values might be redundant if they are generalized in the generalization step. 



%\mostafa{If by semantics you mean the semantics encoded in the generalization hierarchies, I think it is reasonable to assume we have these hierarchies. About close vs far values to be repaired and having added value, there is no real added information here. Even when two dirty values are close, repairing them to their least common ancestor causes loss of information, however it will also resolves inconsistency. Basically, here any repair will cause information loss, if value are further apart (meaning the data is dirtier) more generalization is needed to mask the inconsistency.}


%\fei{Like we discussed, we need to add discussion re. differential privacy and privateClean and distinctions.}

%\mostafa{I added sentences after the problem definition. I think these are different problems although both are about privacy and cleaning.}

%In $R_2$, generalization achieves both the $k$-anonymity privacy requirement and data consistency. In particular, the generalization of Diazepam and Digoxin only resolves the inconsistency w.r.t. $\sigma_2$ and is not necessary for $k$-anonymity. The generalization of AB and MB helps to satisfy $k$-anonymity and the violation of $\sigma_1$. 




%Generalization can also facilitate data repair by transforming inconsistent values to less specific but semantically close values according to a domain generalization hierarchy. In our example, we can generalize $R$ to $R''$ the PRV values in tuples $t_1, t_2, t_7, t_8$ by generalizing the existing values to `Prairies' according to the PRV domain hierarchy shown in  Figure~\ref{fig:general}(a). 


%Example~\ref{ex:k} shows that generalization can serve for both privacy preservation and data repair by masking inconsistencies. Here, we define the problem of clean data publishing to achieve both of these two objectives. For a relation $R$, a set of ICs $\Sigma$ that are falsified by $R$ ($R\not\models \Sigma$), and value $k$ as in $k$-anonymity, the problem of clean data publishing is to find a relation $R'$ that (1) satisfies $\Sigma$, (2) is $k$-anonymous, and (3) minimally generalizes $R$. Here, (1) and (2) concern data consistency and privacy, while (3) restricts the amount of change applied on the given relation $R$ which is a common objective in both data publishing and data repair. The instance $R_2$ in Example~\ref{ex:k} is a possible solution of the problem.

%\blue{PrivateClean is a data cleaning framework addressing a similar problem~\cite{krishnan}. It cleans a differentially private version of the underlying private database that contains dirty values using a limited set of cleaning operations. PrivateClean is different from our problem of clean data publishing. In PrivateClean date repir is delayed and is done over private versions of the original relations. However, here we integrate both cleaning and privacy-aware data publishing in a single task to get higher utility in the result of cleaning. Second, PrivateClean assumes the cleaning process is unknown and only allows a limited cleaning operations that might be used in this process. In our problem, there might be many existing cleaning algorithms that we decide not to apply for the reasons we mentioned in Example~\ref{ex:k}. Finally, the privacy models are different and the differentially private restriction in PrivateClean does not allow high utility cleaning algorithms to run over the private data.}

%\fei{I think there are two problems that need to be solved:}
%\begin{itemize}
%    \item  (i) how to first ``clean'' values that are inconsistent such that they are close and generalization will work; and (ii) deciding on which values to generalize and how much.

%\mostafa{About (i), if we can accurately repair, there is no need to mask violations using generalization. Unless we say only few values can be repaired and then we would like to find those that make generalization more efficient while generalization is still going to mask some violation that are left in the data. This requries a different problem definition with limited repair budget in the first repair phase and then a generalization step to mask errors. Is that the idea?}    

%\mostafa{About (ii), this is already encoded in problem definition. Since there are several instances that satisfy (1) and (2). While (3) captures the restriction on the values to pick for generalization and the extent of generalization over these values.}    

    %\item I think it's also worthwhile to demonstrate in the example a stronger case where by generalizing only (without consideration for cleaning) leads to a very different clustering of tuples than if we were to clean + generalize together, which is a correct solution that uses the FDs (and its semantics) to determine which cells to clean.  This probably requires QI attributes to not be part of the FD attributes.
    
    %\mostafa{I think Table~\ref{tab:r1} and Table~\ref{tab:r1} do exactly what you said. They have different clusterings but Table~\ref{tab:r1} applies cleaning+generalization while Table~\ref{tab:r1} does not clean data beforehand. I did not talk about clustering since it is not part of problem definition and it is about solution.}
%\end{itemize}

